Time After Time: Deep-Q Effect Estimation for Interventions on When and What to do

Problems in fields such as healthcare, robotics, and finance requires reasoning about the value both of what decision or action to take and when to take it. The prevailing hope is that artificial intelligence will support such decisions by estimating the causal effect of policies such as how to treat patients or how to allocate resources over time. However, existing methods for estimating the effect of a policy struggle with \emph{irregular time}. They either discretize time, or disregard the effect of timing policies. We present a new deep-Q algorithm that estimates the effect of both when and what to do called Earliest Disagreement Q-Evaluation (EDQ). EDQ makes use of recursion for the Q-function that is compatible with flexible sequence models, such as transformers. EDQ provides accurate estimates under standard assumptions. We validate the approach through experiments on survival time and tumor growth tasks.

==> Figures/BackwardTime.tex <==
% {\centering
% \begin{figure*}
% \vspace{-15pt}
\begin{minipage}[t]{\linewidth}
\begin{algorithm}[H]
\caption{Backward-in-time Q-Evaluation}
\label{alg:QlearnBackward}

\begin{algorithmic}[1]
    % \small
    \State \textbf{Input}: Trajectories $\{\gH_i\}_{i=1}^{m}$, \\
    \qquad\quad Policy $\pi:\cup_{t=1}^{T}\gX^{t}\times\gA^{t-1} \rightarrow \Delta^{|\gA|}$

    \State $Q_T(\gH_i) = \mathrm{arg}\min_{f}{\sum_{i=1}^{m}{{\left( f(\gH_i) - y_i \right)^2}}}$
    \For{$t \gets T-1$ to $1$}
        \State $\hat{y}_{i} = y_{i,t} + \E_{\tilde{a}_{t+1} \sim \pi(\cdot \vert \gH_{i,t}, \rvx_{i,t+1})}Q_{t+1}(\tgH_{t+1} )$ %$\forall i\in{[N]}$
        \State $Q_t(\gH_t) =
        % \\ \qquad \quad 
\mathrm{arg}\min_{f}\sum_{i=1}^{m}\left( f(\gH_{i,t}) - \hat{y}_i \right)^2$
    \EndFor
    
    \State \textbf{Return} $\{Q_t(\cdot)\}_{t=1}^{T}$
    
\end{algorithmic}
\end{algorithm}
\end{minipage}
% \vspace{-15pt}
% \end{figure*}
% }

==> Figures/ContinuousTimeFQE.tex <==
\begin{algorithm}
\caption{Fitted Q-Evaluation}
\label{alg:FQE}
\begin{algorithmic}[1]
    \State \textbf{Input}: Trajectories $\{\rvx_i, \rva_i, \rvy_i, \rvt_i \}_{i=1}^{N}$, policy $\pi:\cup_{t=1}^{T}\gX^{t}\times\gA^{t-1} \rightarrow \Delta^{|\gA|}$

    \State $Q^t(a_t, \overline{\rvh}_{t}) = 0 \quad \forall t\in{[T]}, a_t, \overline{\rvh}_{t}$
    % $Q^t(a_t, \overline{\rvh}_{t}) = \mathrm{arg}\min_{\vtheta}{\sum_{i=1}^{N}{{\left( f(\rvx_{:T}, \rva_{:T}; \vtheta) - y_{i,T} \right)^2}}}$
    \For{$j \gets 0$ to $n_{\mathrm{updates}}$}
        \State Draw $(\overline{\rvh}_{t,i}, a_{t,i}, y_{i,t}, \overline{\rvh}_{t+1,i})$, where $i\sim \mathrm{Unif}([N]), t\sim \mathrm{Unif}([T])$
        \State $\hat{y}_{i,t} = y_{i,t} + \gamma\E_{a_{t+1}\sim \pi(\overline{\rvh}_{t, i})}f(a_{t+1}, \overline{\rvh}_{t+1, i})$
        \State $\vtheta \gets \vtheta - \eta \nabla_{\theta}\ell(f(a_t, \overline{\rvh}_{t,i}; \vtheta), \hat{y}_{i,y})$
        % \hat{y}_{i,t} = y_{i,t} + \E_{a_{t+1, i} \sim \pi(\overline{\rvh}_{t, i})}Q^T(a_{t+1}, \overline{\rvh}_{t+1, i}) \quad \forall i\in{[N]}$
    \EndFor
    
    \State \textbf{Return} $\{Q^t(\cdot, \cdot)\}_{t=1}^{T}$
\end{algorithmic}
\end{algorithm}

==> Figures/FQE_pseudocode_old.tex <==
\begin{algorithm}
\caption{Fitted Q-Evaluation}
\label{alg:FQE}
\begin{algorithmic}[1]
    \State \textbf{Input}: Trajectories $\{\left(\rvx_i, \rva_i, \rvy_i\right)\}_{i=1}^{N}$, policy $\pi:\cup_{t=1}^{T}\gX^{t}\times\gA^{t-1} \rightarrow \Delta^{|\gA|}$

    \State $Q^t(a_t, \overline{\rvh}_{t}) = 0 \quad \forall t\in{[T]}, a_t, \overline{\rvh}_{t}$
    % $Q^t(a_t, \overline{\rvh}_{t}) = \mathrm{arg}\min_{\vtheta}{\sum_{i=1}^{N}{{\left( f(\rvx_{:T}, \rva_{:T}; \vtheta) - y_{i,T} \right)^2}}}$
    \For{$j \gets 0$ to $n_{\mathrm{updates}}$}
        \State Draw $(\overline{\rvh}_{t,i}, a_{t,i}, y_{i,t}, \overline{\rvh}_{t+1,i})$, where $i\sim \mathrm{Unif}([N]), t\sim \mathrm{Unif}([T])$
        \State $\hat{y}_{i,t} = y_{i,t} + \gamma\E_{a_{t+1}\sim \pi(\overline{\rvh}_{t+1, i})}f(a_{t+1}, \overline{\rvh}_{t+1, i})$
        \State $\vtheta \gets \vtheta - \eta \nabla_{\theta}\ell(f(a_t, \overline{\rvh}_{t,i}; \vtheta), \hat{y}_{i,y})$
        % \hat{y}_{i,t} = y_{i,t} + \E_{a_{t+1, i} \sim \pi(\overline{\rvh}_{t, i})}Q^T(a_{t+1}, \overline{\rvh}_{t+1, i}) \quad \forall i\in{[N]}$
    \EndFor
    
    \State \textbf{Return} $\{Q^t(\cdot, \cdot)\}_{t=1}^{T}$
\end{algorithmic}
\end{algorithm}

==> Figures/FQE_slides.tex <==
% {\centering
% \begin{figure*}
\vspace{-15pt}
\begin{minipage}[t]{\linewidth}
\begin{algorithm}[H]
\caption{Earliest Disagreement Fitted Q-Evaluation}
% \label{alg:FQE_earliest disagreement}

\begin{algorithmic}[1]
    % \State \textbf{Input}: Trajectories $\{\gH_i\}_{i=1}^{m}$, \\
    % \qquad\quad Policy $\lambda_a(\cdot \vert \gH_t), \pi(\cdot \vert \gH_t)$

    \State Initialize $\vtheta$, and $Q_T(\gH_i; \vtheta) = y_i \; \forall i\in{[N]}$
    \For{$K$ iterations}
        \State Draw $t\sim \mathrm{Unif}([0,T])$ and $i \sim \mathrm{Unif}([N])$
        \State  $\tilde{a}_{t+1}\sim \pi(\cdot \vert \gH_{i, t}, \boldsymbol{x}_{i, t+1})$
        \State $\tgH_{t+1} = \gH_{i,t} \cup (\boldsymbol{x}_{i, t+1}, \tilde{a}_{t+1})$
        \State $\hat{y}_{i} = Q_{t+1}(\tgH_{t+1}; \vtheta)$ %$\forall i\in{[N]}$
        \State $\vtheta \leftarrow \vtheta - \eta \nabla_{\vtheta} \left(Q_{t}(\gH_{i,t}; \vtheta) - \hat{y}_i\right)^2$
        % \\ \qquad \quad 
% \mathrm{arg}\min_{f}\sum_{i=1}^{m}\left( f(\gH_{i,t}) - \hat{y}_i \right)^2$
    \EndFor
    
    \State \textbf{Return} $\{Q_t(\cdot; \vtheta)\}$
    
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-15pt}
% \end{figure*}
% }

==> Figures/Lookahead_step.tex <==
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \begin{algorithm}[H]
    \caption{$(\delta, a)$-Sample}
    \label{alg:lookahead}
    \begin{algorithmic}[1]
        \State \textbf{Input}: Trajectory $\rva_i, \rvx_i$ of length $T$, \\ \quad\quad Start time $t\in{[T]}$, \\
        \quad\quad Policy $\pi^*:\cup_{t=1}^{T}\gA^{t-1} \times \gX^{t-1} \rightarrow \Delta^{|\gA|}$
    
        \State $\delta \leftarrow 1$
        \While{$\delta \leq T-t$}
        \State Draw $\tilde{a}_{t+\delta} \sim \pi^*(\cdot \vert \orvh_{i, t+\delta-1})$
        \If{$\tilde{a}_{t+\delta} \neq a_{i,t+\delta}$}
        \State \textbf{Return} $(\delta, \tilde{a}_{t+\delta})$
        \EndIf   
        \State $\delta \leftarrow \delta + 1$
        \EndWhile
        \State \textbf{Return} $(T-t, a_{T})$
    \end{algorithmic}
    \end{algorithm}
\end{minipage}
\begin{minipage}[t]{0.49\linewidth}
\centering
\begin{algorithm}[H]
\caption{FQE with Lookahead}
\label{alg:FQE_lookahead}
\begin{algorithmic}[1]
    \State \textbf{Input}: Trajectories $\{ \rva_i, \rvx_i, y_i\}_{i=1}^{N}$, \\
    \qquad Policy $\pi^*:\cup_{t=1}^{T}\gA^{t}\times\gX^{t-1} \rightarrow \Delta^{|\gA|}$

    \State $Q_t(a_t, \overline{\rvh}_{t}; \vtheta) = 0 \quad \forall t\in{[T]}, a_t, \overline{\rvh}_{t}$
    % $Q^t(a_t, \overline{\rvh}_{t}) = \mathrm{arg}\min_{\vtheta}{\sum_{i=1}^{N}{{\left( f(\rvx_{:T}, \rva_{:T}; \vtheta) - y_{i,T} \right)^2}}}$
    \For{$j \gets 0$ to $n_{\mathrm{updates}}$}
        \State Draw $i,t\sim \mathrm{Unif}([N]\times [T])$
        \State $(\delta, \tilde{a}_{t+\delta}) \leftarrow (\delta, a)\text{-Sample}(\rva_i, \rvx_i, t, \pi^*)$
        \State $\hat{y}_{i,t} =  Q_{t+\delta}(\tilde{a}_{t+\delta}, \orvh_{t+\delta-1, i}; \vtheta)$
        \State $\vtheta \gets \vtheta - \eta \nabla_{\theta}\ell(Q_t(a_t, \overline{\rvh}_{t,i}; \vtheta), \hat{y}_{i,t})$
    \EndFor
    
    \State \textbf{Return} $\{Q_t(\cdot, \cdot; \vtheta)\}_{t=1}^{T}$
\end{algorithmic}
\end{algorithm}
\end{minipage}

% \begin{algorithm}
% \caption{GetNextTimeAndAction}
% \label{alg:lookahead}
% \begin{algorithmic}[1]
%     \State \textbf{Input}: Trajectory $\rva_i, \rvy_i, \rvn_i$ of length $T$, start time $t\in{[T]}$
%     \State \quad \quad \quad ~  policy $\pi^*:\cup_{t=1}^{T}\gA^{t-1} \times \gY^{t-1} \rightarrow \Delta^{|\gA|}$, schedule $\lambda^*:\cup_{t=1}^{T-1} \gA^{t-1} \times \gY^{t-1} \rightarrow [0,1]$

%     \State $\delta \leftarrow 1$
%     \While{$\delta < T-t$}
%     \State $p \leftarrow P_{\pi^*,\lambda^*}(a_{i,t+\delta}, n_{i, t+\delta} \vert \orva_{i, t+\delta-1}, \orvn_{i, t+\delta-1})$
%     \State Draw $B\in{\{0,1\}}$ with success probability $1-p$
%     \If{$B=1$}
%     \State Return $\delta$
%     \EndIf   
%     \State $\delta \leftarrow \delta + 1$
%     \EndWhile
%     \State \textbf{Return} $\delta$
% \end{algorithmic}
% \end{algorithm}
% \begin{algorithm}
% \caption{FQE with Lookahead}
% \label{alg:FQE_lookahead}
% \begin{algorithmic}[1]
%     \State \textbf{Input}: Trajectories $\{ \rva_i, \rvy_i, \rvn_i\}_{i=1}^{N}$, policy $\pi^*:\cup_{t=1}^{T}\gA^{t}\times\gY^{t-1} \rightarrow \Delta^{|\gA|}$

%     \State $Q^t(a_t, \overline{\rvh}_{t}) = 0 \quad \forall t\in{[T]}, a_t, \overline{\rvh}_{t}$
%     % $Q^t(a_t, \overline{\rvh}_{t}) = \mathrm{arg}\min_{\vtheta}{\sum_{i=1}^{N}{{\left( f(\rvx_{:T}, \rva_{:T}; \vtheta) - y_{i,T} \right)^2}}}$
%     \For{$j \gets 0$ to $n_{\mathrm{updates}}$}
%         \State Draw $(\overline{\rvh}_{t,i}, a_{t,i})$, where $i\sim \mathrm{Unif}([N]), t\sim \mathrm{Unif}([T])$
%         \State $\delta \leftarrow \mathrm{GetNextTimeAndAction}(\{\rva_i, \rvy_i, \rvn_i\}, t, \pi^*, \lambda^*)$
%         \State $\hat{y}_{i,t} = y_{i,t} + \E_{a_{t+\Delta}\sim \pi(\overline{\rvh}_{t+\delta-1, i})}f_{t+\delta}(a_{t+\delta}, \overline{h}_{t+\delta-1, i})$
%         \State $\vtheta \gets \vtheta - \eta \nabla_{\theta}\ell(f_t(a_t, \overline{\rvh}_{t,i}; \vtheta), \hat{y}_{i,t})$
%     \EndFor
    
%     \State \textbf{Return} $\{Q^t(\cdot, \cdot)\}_{t=1}^{T}$
% \end{algorithmic}
% \end{algorithm}

==> sections/4_estimation_old.tex <==
% \section{Methods for Estimating When and What to do}
% We are now in place to present estimation methods for $\E_{P}[Y \vert \gH_t]$. The generative approach for 
% \subsection{Estimation with Autoregressive Models}
% Assume we observe the history $\gH_{t_i}$ where $t_i$ is the time of the $i$-th event in a trajectory. Denote $T_{x, i+1}, T_{a, i+1}$ as random variables for the next state observation time and next treatment time after $t_i$ respectively.
% \begin{itemize}
%     \item Fit $P_{\vtheta}(T^x_{ \mathrm{next},i}, X_{\mathrm{next}} \vert \gH_{t_i}, T^x_{\mathrm{next}, i} < T^a_{\mathrm{next}, i})$
%     \item Assume we are given access to a procedure that samples $T^a_{\mathrm{next}, i}$ from $P_{\lambda}(T^a_{\mathrm{next}} \vert \gH_{t_i}, T^a_{\mathrm{next}, i} < T^x_{\mathrm{next}, i})$, where we recall $P_{\lambda}$ is the interventional distribution.
%     \item Note that under the no-instantaneous effect assumption, the likelihood of the next event being an action at time $t_i + \delta$ is
%     \begin{align} \label{eq:intense_a_next}
%     \lambda_{a}(t+\delta)\exp\left\{ -\int_{t}^{t+\delta} \lambda_{\bullet}(s \vert \gH_{s}=\gH_{t}) d s \right\},
%     \end{align}
%     and respectively for $\lambda_{x}(t+\delta)$.
%     We claim that sampling $T^a_{\mathrm{next}, i} \wedge T^x_{\mathrm{next}, i}$
%     results in a process that gives the correct likelihoods, under the assumption of no instantaneous effects.
%     First, note that for any $\delta > 0$, $P_{\lambda}(T^a_{\mathrm{next}, i} \wedge T^x_{\mathrm{next}, i} = T^a_{\mathrm{next}, i} = t_i+\delta) = P_{\lambda}(T^a_{\mathrm{next}} = t+\delta \vert \gH_{t_i}, t_i+\delta < T^x_{\mathrm{next},i})P_{\lambda}(t_{i}+\delta < T^{x}_{\mathrm{next}, i})$. The first term is
%     \begin{align*}
%     P_{\lambda}(T^a_{\mathrm{next}} = t+\delta \vert \gH_{t_i}, t_i+\delta < T^x_{\mathrm{next},i}) = \lambda_{a}(t+\delta)\exp\left\{ -\int_{t}^{t+\delta} \lambda_{a}(s \vert \gH_{s}=\gH_{t}) d s \right\}
%     \end{align*}
%     whereas the second is
%     \begin{align*}
%     P_{\lambda}(T^x_{\mathrm{next}} > t+\delta \vert \gH_{t_i}, t_i+\delta < T^x_{\mathrm{next},i}) = \exp\left\{ -\int_{t}^{t+\delta} \lambda_{x}(s \vert \gH_{s}=\gH_{t}) d s \right\}
%     \end{align*}
% \end{itemize}
% Multiplying them, we get the correct likelihood term in \cref{eq:intense_a_next}. Hence our sampling procedure matches the interventional distribution $P_{\lambda}$ of the next event time and type.
\section{Model Free Off-Policy Evaluation for Decision Point Processes} \label{sec:method}
To estimate $\E_{P}[ Y \vert \gH_t ]$ for times $t$ and $\gH_t$ that overlap with $P_\obs$, we express the expectation recursively as a function of expectations $\E_{P}[Y \vert \tgH_{t+\delta} ]$ for some $\delta > 0$ and trajectory $\tgH$. Then, assuming that expectations at times larger than $t$ have been learned correctly, this recursive expression allows us to propagate information for conditioning on earlier histories. Let us describe this solution in more detail, as applied in the context of $Q$-evaluation. 

% This type of dynamic programming, by going backwards in time, is a well known solution for discrete time problems. Thus, we first describe it and then address the challenges that arise when adapting it to continuous time.

\begin{wrapfigure}{r}{0.55\textwidth}
% rr: should the algorithm have an expectation in line 5
% yw: you mean that instead we could just sampling a single $\tilde{a}_{t+1}$ from the policy and drop the expectation, i.e. $\hat{y}_i = y_{i,t} + Q_{t+1}(\tilde{H}_{t+1})$?
% if so, we can do that 
    \input{Figures/BackwardTime}
\end{wrapfigure}
\textbf{Fitted Q evaluation (FQE) in discrete time.} Q-evaluation relies on the tower property of conditional expectations, given below in \cref{eq:tower}. In discrete time decision processes, where we consider $\delta=1$, the property suggests a dynamic programming solution that we lay out in \cref{alg:QlearnBackward} \citep{le2019batch, watkins1992q}. Here, $\gH_t$ includes all actions and observations up to and including time $t$, and 
since they occur simultaneously, there are exactly $t$ of each. 
% rr: tilde{H} is not clear. I think you should do something like H_{t+1}[\tilde{a}_{t+1}] or something like H_t + x_{t+1} + \tilde{a}_{t+1}
$\tgH_{t+1}$ is defined in the same manner, except that it includes $\tilde{a}_{t+1}$ sampled from the target policy $\pi$.
\begin{align} \label{eq:tower}
\E_{P}\left[Y \vert \gH_t \right] = \E_{\tgH_{t+\delta}\sim P(\cdot \vert \gH_t)}\left[\E_{P}\left[ Y \vert \tgH_{t+\delta} \right] \right],
\end{align}
An attractive property of this algorithm is that it is \emph{model-free}. That is, to form the label $\hat{y}_i$ we only need to sample $\tilde{a}_{t+1}$ from our target policy $\pi$, while a model of $P(\rvx_{t+1} \vert \gH_t)$ is not necessary.


Under favorable conditions of accurate optimization over a sufficiently expressive hypothesis class and an arbitrarily large datasets, \cref{alg:QlearnBackward} returns correct estimates. 
% rr: this looks odd because i want to split out the Y_{t}
This is because if we fix $Q_{t+1}(\gH_{t+1})$ and assume that it accurately estimates $\E_{P}[ \sum_{s\geq t+1} Y_s \vert \gH_{t+1} ]$, then, the minimizer of the regression in the algorithm is the conditional expectation, which equals $\E_{P}[ \sum_{s\geq t} Y_s \vert \gH_{t} ]$ according to \cref{eq:tower}.
The model-free solution is enabled by the equality $P(\rvx_{t+1} \vert \gH_t) = P_{\obs}(\rvx_{t+1} \vert \gH_t)$, which validates the use of $\rvx_{i, t+1}$ to form $\hat{y}_i$. In practical implementation, we apply gradient steps on randomly drawn times and training samples instead of walking backward in time from $T$ to $1$.
% and we can use our training trajectories to approximate this sampling. To sample $a_{t+1}$ we need to sample from our target policy $\pi^*(\cdot \vert \orvh_{t+1})$, which we assume is possible and efficient. This forms the basis of FQE going backwards in time in \cref{alg:QlearnBackward}
Crucially, for $\delta > 1$, e.g. $\delta=2$, we have $P(\rvx_{t+2} \vert \gH_t) \neq P_{\obs}(\rvx_{t+2}\vert \gH_t)$. Hence an algorithm based on \cref{eq:tower} will either be model-based, or resort to using solutions such as products of importance weights that suffer from high variance \citep{precup2000eligibility, hallak2016generalized}, or restrict the problem, e.g., by discounting rewards \citep{munos2016safe, harutyunyan2016q, precup2000eligibility}. \\

\textbf{Challenges in application to continuous time.} Moving to continuous time, the tower property turns into a differential equation, and solving it requires tools that go beyond the common FQE solution, e.g. \citep{jia2023q}. Regressing to an outcome that is arbitrarily close to the observation at time $t$ is ill-defined. While we may work under a fine discretization of time, this approach is wasteful, as a single update in the minimization for estimating $Q_t$ takes into account the development of the process in the interval $[t, t+\delta]$, and for small values of $\delta$ this will usually yield a very small change to the estimate. Hence, intuitively, when updating $Q_t$, we would like to use estimates of $Q_{t+\delta}$ for a large $\delta$. As explained above, this is seemingly difficult to achieve in a model-free fashion. However, for point processes, since the number of decisions over $[0,T]$ is countable, it seems plausible that a simple and efficient dynamic programming solution can be devised. In what follows, this is what we present.

\subsection{\ours{}: Fitted Q-Evaluation for Decision Point Processes via Earliest Disagreement Times}
% rr: this paragraph needs to be rewritten. i didn't get much from it. what points do you want to make?
Consider the following intuition. Assume we observe the entire trajectory of a patient treated by doctor $c$, who practices policy $\lambda_a^{\obs}$. We wish to reason about the patient's outcome had they, from time $t$ onwards, been treated by doctor $\tilde{c}$ who practices policy $\lambda_a$. With $\gH_t$ as the patient history up to time $t$, we look at $c$'s treatment decisions and find the first time in the trajectory, say $t+\delta$, where $\tilde{c}$ would have acted differently from $c$. It seems reasonable to assume the following: the expected outcome of a patient with history $\gH_t$, had they been treated with $\lambda_a$ from time $t$ onwards, would be similar to the expected outcome of patients treated with $\lambda_a$ from time $t+\delta$, with history similar to $\gH_{t+\delta}$. This is because we have no reason to assume $\gH_u$ for $u\in{[t, t+\delta)}$ would have changed under $\tilde{c}$'s policy $\lambda$, as it agreed with $\lambda_{\obs}$ up until that time point. The time $t+\delta$ is the earliest disagreement time between the two policies.\footnote{Under our formulation, with probability $1$, this time will be the first treatment after $t$ drawn by one of the policies. This is because we choose to work with continuous and differentiable compensators $\Lambda^a,\Lambda^a_{\obs}$ (a compensator is $\Lambda$ such that $d\Lambda$ is the intensity $\lambda$). Yet this is a technical convenience, and we can also form our arguments under conditions where treatment times have a non-zero probability to coincide, and the arguments about first disagreement times will stay in tact.} Let us now formalize this intuition and use it to derive an estimation method based on fitted $Q$-evaluation.

\begin{comment}
Moving to continuous time, the tower property turns into a differential equation, and solving it requires tools that go beyond the standard FQE solution, e.g. \citep{jia2023q}, as regressing to an outcome that is arbitrarily close to the observation at time $t$ is ill-defined. To keep using simple methods such as FQE, one can always work under a fine discretization of the space. Yet this is wasteful, as a single update in the minimization for estimating $\hat{Q}_t$ takes into account the development of the process in the interval $[t, t+\delta]$, and for small values of $\delta$ this will usually yield a very small change to the estimate. Hence in updating $\hat{Q}_t$, we would like to use estimates of $\hat{Q}_{t+\delta}$ in some later time, but in a model-free fashion. We will choose $q_t(\delta, \tilde{a}_{t+\delta} \vert a_T, \orvh_T)$ that given an observed trajectory $(a_t, \orvh_T)$ and time $t$, defines a distribution over lookahead times for which we will use $\hat{Q}_{t+\delta}$ in the FQE updates. That is, we will choose a distribution such that the following identity is satisfied,
\begin{align} \label{eq:tower_lookahead}
\E_{\pi^*}\left[ Y \vert a_t, \orvh_t \right] = \E_{\urvh_{t+1}\sim P_{\pi}(\cdot \vert a_t, \orvh_t)}\left[ \E_{ \delta, \tilde{a}_{t+\delta}\sim  q_t(\cdot \vert a_T, \orvh_T)}\left[\E_{\pi^*}\left[Y \vert \tilde{a}_{t+\delta}, \orvh_{t+\delta}\right]\right]\right].
\end{align}
Again, the left hand side is our target quantity, while the inner expectations of the right hand side are similar to that of \cref{eq:tower} when we fix all the history up to time $t+\delta$, and it boils down to. The outer expectation is the important part, where future of trajectories is sampled over the observed distribution, and a value $\delta$ is sampled conditioned on the entire training trajectory. This $\delta$ determines the look ahead time which we will use in our Q-evaluation, as depicted in \cref{alg:todo}. Notably, the identity in \cref{eq:tower_lookahead} does not hold for general choices of $p_t$, and this distribution has to be chosen carefully. We now turn to describe our construction, prove its validity, and this will be incorporated into the FQE algorithm to obtain our lookahead algorithm which we summarize in \cref{alg:FQE_lookahead}.
\end{comment}
% $\tPr_t^a(N^a(du) \vert \tgH_u)$
\begin{definition} \label{def:future_dist}
Consider a fixed trajectory $\gH$ sampled from $P_{obs}$ and a time $t\in{[0,T)}$, we define a marked point process $\tPr_t^a$ on the interval $(t, T]$ with intensity function $\lambda^a(u \vert \gH_u)$ and mark distribution $\pi(A_u \vert \gH_u)$. We use the notation $\tgH^a_u$ to denote trajectories sampled from $\tPr_t^a$ up to time $u$ and define $\tgH_u := \gH^\rma_{t}\cup \tgH^{\rma}_u \cup\gH_u^{\rmx,\rmy}$ for $u\in{(t, T]}$. For the trajectory $\tgH$ we define $\delta_{\tgH}(t) = \min\{u-t : u > t, (u,\cdot)\in{\tgH^a}\}$,\footnote{In case the set is empty we define the minimum as $T-t$} as the first jump time of a trajectory sampled from $\tPr_t^a(\cdot \vert \gH_t )$, and likewise $\delta_{\gH}(t)$ for the observed trajectory $\gH$ instead of $\tgH$.
\end{definition}
Here, $\tgH$ holds the decisions after time $t$ sampled from our target policy, conditioned on the features observed in $\gH$. Notice that to obtain $\tgH$, we only need to sample from the target policy $\lambda^a$ and not from $\lambda^{x,y}$, as $\gH$ can be taken from our training set sampled from $P_\obs$. Our model-free evaluation method is thus based on the following result, which expresses our estimand as an expectation over the trajectories $\tgH$.
% \begin{theorem}
% Let $P, P_\obs$ be multivariate marked decision point processes, $t\in{[0, T)}$, and $\gH_t$ a list of events up to time $t$. For any trajectory $\gH$, we let $\tPr_t^a(\cdot \vert \gH), \delta_{\tgH}(t), \delta_{\gH}(t)$ as in \cref{def:future_dist}. Under assumptions $1$-$3$, we have that
% \begin{align} \label{eq:expectation_identity}
% \E_{P}\left[ Y \vert \gH_{t} \right] = 
% \E_{\gH \sim P_{\obs}(\cdot \vert \gH_{t})}\left[{\E_{\tgH\sim \tPr_t^a(\cdot \vert \gH)}\left[\E_{P}\left[ Y \big \vert \tgH_{t+\delta_\gH(t) \wedge \delta_{\tgH} (t)} \right]\right]}\right].
% \end{align}
% \label{thm:expectation_identity}
% \end{theorem}
\begin{restatable}{thm}{expectationid}
\label{thm:expectation_identity}
Let $P, P_\obs$ be multivariate marked decision point processes, $t\in{[0, T)}$, and $\gH_t$ the trajectory up to time $t$. For any trajectory $\gH$, we let $\tPr_t^a(\cdot \vert \gH), \delta_{\tgH}(t), \delta_{\gH}(t)$ as in \cref{def:future_dist}. Under Assumptions~\ref{assump:ignor} and \ref{assump:overlap}, we have that
\begin{align} \label{eq:expectation_identity}
\E_{P}\left[ Y \vert \gH_{t} \right] = 
\E_{\gH \sim P_{\obs}(\cdot \vert \gH_{t})}\left[{\E_{\tgH\sim \tPr_t^a(\cdot \vert \gH)}\left[\E_{P}\left[ Y \big \vert \tgH_{t+\delta_\gH(t) \wedge \delta_{\tgH} (t)} \right]\right]}\right].
\end{align}
\end{restatable}
\textbf{Takeaways from \Cref{thm:expectation_identity}.}  
% rr: it's helpful to go from the tower property of the expectation to the update rule in the main text here
Our method, described in \cref{alg:FQE_earliest disagreement}, is an empirical version of \cref{eq:expectation_identity} akin to FQE being the empirical version of the tower property of conditional expectations, \cref{eq:tower}, in discrete time.
An analogous result to ours holds for discrete-time decision processes, where \ours{} does not reduce to FQE and instead it bears some resemblance to the eligibility traces approach of \citet{precup2000eligibility}. We provide this result in the appendix for completeness but focus here on the point process case, as this is our main motivation and where the earliest disagreement approach is most fruitful. 
% rr:  this sentence should remove the algorithm mention because you already note the walk backward in time earlier for algorithm 1
Note that \Cref{alg:FQE_earliest disagreement} does not go backward in time as \Cref{alg:QlearnBackward} and follows a more practical version of FQE, e.g. \citep[alg.~1]{le2019batch}, which updates the $Q$ functions at randomly drawn times across the trajectory according to the dynamic program implied by the towered expectations identity.
\begin{figure}
\input{Figures/ED_FQE}  
\end{figure}
We draw an update time and trajectory uniformly from the interval of the process and the training set accordingly, although other distributions on time may be considered, as well as batched optimization over trajectories. Another notable point is that updates are made upon disagreement in \emph{treatments}, and the trajectory in time $(t, t+\delta]$ may include multiple observations and outcomes $\rvx, \rvy$. This is desirable in cases such as intensive care unit data, where some features like vitals are continuously monitored (e.g., blood pressure), while decisions, such as changing medication dosages, occur on a more coarse timescale. The algorithm will then perform updates on the coarser time scale instead of the finer one.
% \textbf{TODO:} explain how to sample from a given policy (optional: currently I think we'll experiment with deterministic dynamic policies, since they are simple and intuitive. They do not exactly match the theory, but I think it is not a super-crucial caveat at this time), describe an architecture with continuous time positional embeddings, and perhaps with predictions of the next action and its time



==> sections/6_conclusion.tex <==
\section{Conclusions, Future Work and Limitations}
Limitations that should be addressed in future work include dealing with censoring and allowing for optimization of policies. Ensuring overlap is a major challenge in such extensions and also in the current work since verifying overlap in a statistically efficient manner is quite challenging.

We also experiment with rather simple and common architectures here, so there is room for improvement by considering different architectures for irregularly sampled data in off-policy evaluation and effect estimation.

==> sections/lem2_proof_backup.tex <==
    \begin{proof} [Proof of \cref{lem:k_stops_lemma}]
For $d=1$, \cref{eq:k_stops_lemma} is exactly \cref{eq:alg_expect_general} which we already proved in \cref{lem:one_stop_lemma}, and we will proceed by induction. Assume for some $d-1>1$ that \cref{eq:k_stops_lemma} holds, and shorten the notation $t+\delta^{d-1}_{\tgH^v}(t)$ to $t_{d-1}$ from now on for convenience. Using \cref{lem:one_stop_lemma} again, it also holds that
% \delta^d_v, \delta^{a_{\obs}},  \delta^a
\begin{align} \label{eq:process_proof_eq1}
\E_{P}\left[ Y \vert \gH_{t_{d-1}} \right] = \nonumber\\
\E_{\gH \sim P_{\obs}(\cdot  \vert \gH_{t_{d-1}})}\Big[ \\
\E_{\tgH \sim \tPr(\cdot \vert \gH)}\Big[ & \mathbf{1}\big[\delta^a(t_{d-1}) < \delta^v(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\big]\E_P\left[ Y \vert \gH_t \cup (t+\delta^a(t_{d-1}), a) \right] + \nonumber \\
 & \mathbf{1}\big[\delta^v(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\big]\E_P\left[ Y \vert \gH_t \cup (t+\delta^v(t_{d-1}), v) \right] + \nonumber \\ 
 & \mathbf{1}\big[\delta^{a_{\obs}}(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^v(t_{d-1})\big]\E_P\left[ Y \vert \gH_{t+\delta^{a_{\obs}}(t_{d-1})} = \gH_t \right] + \nonumber \\
 & \mathbf{1}\big[\delta^{a_{\obs}}(t_{d-1})\wedge\delta^a(t_{d-1})\wedge \delta^v(t_{d-1}) > T-t\big]\E_P\left[ Y \vert \gH_{T} = \gH_t \right]\Big]\Big]
\end{align}
Now let us write down the induction hypothesis,
\begin{align} \label{eq:process_proof_induction_hypo}
\E_P[Y \vert \gH_t] &= \E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}\Big[ \\
&\sum_{k=1}^{d-1} \Big( \mathbf{1}\big[\delta^{k-1}_{\gH^v}(t) \leq \delta_{\gH^a}(t) < \delta^{k}_{\gH^v}(t) \wedge \delta_{\obs}^{\gH^a}(t) \wedge T-t \big] \E_{P}\big[Y \vert \tgH_{t+\delta_{\gH^a}(t)}\big] \nonumber \\
&+\mathbf{1}\big[\delta^{k-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) < t+\delta^{k}_{\gH^v}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \E_{P}\big[Y \vert \tgH_{t+\delta_{\gH^{\obs}_a}(t)}\big] \nonumber \\
&+\mathbf{1}\big[ T-t < \delta^k_{\gH^v}(t)\wedge \delta_{\obs}^{\gH^a}(t)\wedge \delta_{\gH^a}(t) \big] \E_{P}[Y \vert \gH_T=\gH_t]\Big)\nonumber \\
&+\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \E_{P}\big[Y \vert \tgH_{t+\delta^{d-1}_{\gH^v}(t)}\big] 
\Big]\bigg] \nonumber
\end{align}
Since the argument of the expectation $\E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}[\cdot]]$ only contains events that occur in $(t, t+\delta^{d-1}_{v}(t)]$, we can condition the inner expectation on $\gH$ stopped at $t+\delta^{d-1}_{v}(t)$, i.e. $\E_{\tgH_{t+\delta^{d-1}_v(t)}\sim\tPr^a_t(\cdot \vert \gH_{t+\delta^{d-1}_{v}(t)})}[\cdot]$ (this also requires noticing that $\tPr^a_t$ samples increments in $(t, t+\delta^{d-1}_v(t)]$ independently of events that occur after $t+\delta^{d-1}_v(t)$). Now for a similar reason we can sample $\gH$ from $P_{\obs}$ and stop at the $d-1$-th jump of $N_v$.
Overall, below we replace $\E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}[\cdot]]$ with $\E_{\gH_{t+\delta^{d-1}_{\gH^v}(t)}\sim P_{\obs}(\cdot \vert \gH_t)}[\E_{\tgH_{t+\delta^{d-1}_{\gH^v}(t)}\sim\tPr^a_t(\cdot \vert \gH_{t+\delta^{d-1}_{\gH^v}(t)})}[\cdot]]$ in the last summand taken from \cref{eq:process_proof_induction_hypo} and change again to the notation $t_{d-1}$ used at the beginning of the proof to make terms a bit more compact.
\begin{align*}
    &\E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}\Big[\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T \big] \E_{P}\big[Y \vert \tgH_{t+\delta^{d-1}_{\gH^v}(t)}\big] 
\Big]\bigg] \\
=&\E_{\gH_{t+\delta^{d-1}_{\gH^v}(t)}\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH_{t+\delta^{d-1}_{\gH^v}(t)}\sim\tPr^a_t(\cdot \vert \gH_{t+\delta^{d-1}_{\gH^v}(t)})}\Big[ \\
&\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T \big] \E_{P}\big[Y \vert \gH_{t+\delta^{d-1}_{\gH^v}(t)}\big] 
\Big]\bigg] \\
=&\E_{\gH_{t_{d-1}}\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH_{t_{d-1}}\sim\tPr^a_t(\cdot \vert \gH_{t_{d-1}})}\Big[ \mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T \big] \E_{P}\big[Y \vert \gH_{t_{d-1}}\big] 
\Big]\bigg].
\end{align*}
The first transition also replaces conditioning on $\tgH_{t+\delta^{d-1}_v(t)}$ with $\gH_{t+\delta^{d-1}_v(t)}$ which holds since when $\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T \big] = 1$ we know that $N_a, N_a^{\obs}$ do not jump in $(t, t_{\delta^{d-1}_{\gH^v}(t)}]$, and hence these histories are equal. Next we plug-in \cref{eq:process_proof_eq1} into the last item.
\begin{align*}
&\E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}\Big[\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \E_{P}\big[Y \vert \tgH_{t+\delta^{d-1}_{\gH^v}(t)}\big] 
\Big]\bigg] = \\
&\E_{\gH_{t_{d-1}}\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH_{t_{d-1}}\sim\tPr^a_t(\cdot \vert \gH_{t_{d-1}})}\Big[ \mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \cdot \\
&\quad \E_{\gH \sim P_{\obs}(\cdot  \vert \gH_{t_{d-1}})}\Big[ \E_{\tgH \sim \tPr^a_{t_{d-1}}(\cdot \vert \gH)}\Big[ \\
&\quad \mathbf{1}\big[\delta^a(t_{d-1}) < \delta^v(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_t \cup (t+\delta^a(t_{d-1}), a) \right] + \nonumber \\
& \quad \mathbf{1}\big[\delta^v(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_t \cup (t+\delta^v(t_{d-1}), v) \right] + \nonumber \\ 
& \quad \mathbf{1}\big[\delta^{a_{\obs}}(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^v(t_d-1) \wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{t+\delta^{a_{\obs}}(t_{d-1})} = \gH_{t_{d-1}} \right] + \nonumber \\
& \quad \mathbf{1} \big[\delta^{a_{\obs}}(t_{d-1})\vee \delta^a(t_{d-1}) \vee \delta^v(t_{d-1}) > T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{T} = \gH_{t_{d-1}} \right]\Big] 
\Big]\bigg]
\end{align*}
Next we pull the expectations $\E_{\gH \sim P_{\obs}(\cdot  \vert \gH_{t_{d-1}})}[ \E_{\tgH \sim \tPr^a_{t_{d-1}}(\cdot \vert \gH)}[\cdot]]$ outside.
\begin{align*}
&\E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}\Big[\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \E_{P}\big[Y \vert \tgH_{t+\delta^{d-1}_{\gH^v}(t)}\big] 
\Big]\bigg] = \\
&\E_{\gH_{t_{d-1}}\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[ \E_{\gH \sim P_{\obs}(\cdot  \vert \gH_{t_{d-1}})} \Big[ \E_{\tgH \sim \tPr^a_{t_{d-1}}(\cdot \vert \gH)}\Big[\E_{\tgH_{t_{d-1}}\sim\tPr^a_t(\cdot \vert \gH_{t_{d-1}})}\Big[ \\
&\quad \mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \cdot \Big( \\
&\quad \mathbf{1}\big[\delta^a(t_{d-1}) < \delta^v(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_t \cup (t+\delta^a(t_{d-1}), a) \right] + \nonumber \\
& \quad \mathbf{1}\big[\delta^v(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_t \cup (t+\delta^v(t_{d-1}), v) \right] + \nonumber \\ 
& \quad \mathbf{1}\big[\delta^{a_{\obs}}(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^v(t_{d-1}) \wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{t+\delta^{a_{\obs}}(t_{d-1})} = \gH_{t_{d-1}} \right] + \nonumber \\
& \quad \mathbf{1} \big[\delta^{a_{\obs}}(t_{d-1}) \vee \delta^a(t_{d-1}) \vee \delta^v(t_{d-1}) > T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{T} = \gH_{t_{d-1}} \right] \Big) \Big] 
\Big] \Big] \bigg] = \\
&\E_{\gH \sim P_{\obs}(\cdot \vert \gH_t)}\bigg[  \E_{\tgH \sim \tPr^a_{t}(\cdot \vert \gH)}\Big[ \\
&\quad \mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \cdot \Big( \\
&\quad \mathbf{1}\big[\delta^a(t_{d-1}) < \delta^v(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_t \cup (t+\delta^a(t_{d-1}), a) \right] + \nonumber \\
& \quad \mathbf{1}\big[\delta^v(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_t \cup (t+\delta^v(t_{d-1}), v) \right] + \nonumber \\ 
& \quad \mathbf{1}\big[\delta^{a_{\obs}}(t_{d-1}) < \delta^a(t_{d-1})\wedge \delta^v(t_{d-1}) \wedge T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{t+\delta^{a_{\obs}}(t_{d-1})} = \gH_{t_{d-1}} \right] + \nonumber \\
& \quad \mathbf{1} \big[\delta^{a_{\obs}}(t_{d-1})\vee \delta^a(t_{d-1}) \vee \delta^v(t_{d-1}) > T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{T} = \gH_{t_{d-1}} \right] \Big) \Big] \bigg].
\end{align*}
Now it is easy to simplify the multiples of indicator functions as conjunctions, for instance by observing that,
\begin{align*}
    &\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \cdot \\ 
 &\quad \mathbf{1}\big[\delta^a(t_{d-1}) < \delta^v(t_{d-1})\wedge \delta^{a_{\obs}}(t_{d-1})\wedge T-t_{d-1}\big] = 
    \mathbf{1}\big[ \delta_{v}^{d-1} \leq \delta^a(t) \leq \delta^{d}_v \wedge \delta^{a_{\obs}}(t) \wedge T-t \big].
\end{align*}
Simplifying the rest of the terms in a similar manner we arrive at
\begin{align*}
&\E_{\gH\sim P_{\obs}(\cdot \vert \gH_t)}\bigg[\E_{\tgH\sim\tPr^a_t(\cdot \vert \gH)}\Big[\mathbf{1}\big[\delta^{d-1}_{\gH^v}(t) \leq \delta_{\obs}^{\gH^a}(t) \wedge \delta_{\gH^a}(t) \wedge T-t \big] \E_{P}\big[Y \vert \tgH_{t+\delta^{d-1}_{\gH^v}(t)}\big] 
\Big]\bigg] = \\
&\E_{\gH \sim P_{\obs}(\cdot \vert \gH_t)}\bigg[  \E_{\tgH \sim \tPr^a_{t}(\cdot \vert \gH)}\Big[ \\
&\quad \mathbf{1}\big[\delta^{d-1}_{v}(t) \leq \delta^a(t) \leq \delta^d_v(t) \wedge \delta^{a_{\obs}}(t)\wedge T-t\big]\cdot\E_P\left[ Y \vert \gH_{t_{d-1}} \cup (t+\delta^a(t), a) \right] + \nonumber \\
&\quad \mathbf{1}\big[\delta^{d}_{v}(t) \leq \delta^a(t) \wedge \delta^{a_{\obs}}(t)\wedge T-t\big]\cdot\E_P\left[ Y \vert \gH_{t_{d-1}} \cup (t_{d-1}+\delta^v(t_{d-1}), v) \right] + \nonumber \\
&\quad \mathbf{1}\big[\delta^{d-1}_v(t) \leq \delta_{\obs}^{a}(t) < \delta^{d}_v(t) \wedge \delta^a(t) \wedge T-t\big]\cdot\E_P\left[ Y \vert \gH_{t_{d-1}} \cup (t+\delta^{a_{\obs}}(t), a) \right] + \nonumber \\
&\quad \mathbf{1} \big[\delta^{a_{\obs}}(t_{d-1})\vee \delta^a(t_{d-1}) \vee \delta^v(t_{d-1}) > T-t_{d-1}\big]\cdot\E_P\left[ Y \vert \gH_{T} = \gH_{t_{d-1}} \right] \Big] \bigg] = \\
&\E_{\gH \sim P_{\obs}(\cdot \vert \gH_t)}\bigg[  \E_{\tgH \sim \tPr^a_{t}(\cdot \vert \gH)}\Big[ \\
&\quad \mathbf{1}\big[\delta^{d-1}_{v}(t) \leq \delta^a(t) \leq \delta^d_v(t) \wedge \delta^{a_{\obs}}(t)\wedge T-t\big]\cdot\E_P\left[ Y \vert \gH_{t_{d-1}} \cup (t+\delta^a(t), a) \right] + \nonumber \\
&\quad \mathbf{1}\big[\delta^{d}_{v}(t) \leq \delta^a(t) \wedge \delta^{a_{\obs}}(t)\wedge T-t\big]\cdot\E_P\left[ Y \vert \gH_{t_{d-1}} \cup (t_{d-1}+\delta^v(t_{d-1}), v) \right] + \nonumber \\
&\quad \mathbf{1}\big[\delta^{d-1}_v(t) \leq \delta_{\obs}^{a}(t) < \delta^{d}_v(t) \wedge \delta^a(t) \wedge T-t\big]\cdot\E_P\left[ Y \vert \gH_{t_{d-1}} \cup (t+\delta^{a_{\obs}}(t), a) \right] + \nonumber \\
&\quad \mathbf{1} \big[\delta^{a_{\obs}}(t)\vee \delta^a(t) \vee \delta^{d}_v(t) > T-t\big]\cdot\E_P\left[ Y \vert \gH_{T} = \gH_{t_{d-1}} \right] \Big] \bigg].
\end{align*}
Plugging this into the induction hypothesis at \cref{eq:process_proof_induction_hypo} we arrive at the desired identity.
\end{proof}

==> sections/old_1_introduction.tex <==
\section{Introduction}
Sequential decision making is ubiquitous across various domains, including healthcare, finance, and beyond. In hospitals, medical professionals administer treatments based on the evolving observations of a patient's condition; in financial markets, traders execute orders based on sequential information flows. Algorithmic decision support systems, therefore, can play a pivotal role in such processes. The essence of these systems often revolves around answering causal questions, which are fundamental to predicting and influencing outcomes.

Consider the scenario of a doctor and patient forming a preventative treatment strategy for Atherosclerotic Cardiovascular Disease (ASCVD). The guidelines of the American Heart Association recommend calculating a 10-year risk score assessing the probability of developing ASCVD, and courses of treatment are recommended according to risk groups formed on the basis of these probabilities. At first glance, this might seem straightforward—calculate the risk score using existing models and proceed based on the result. However, other considerations may come into play, such as patients preferring to start treatment later, e.g. on their next yearly visit due to possible side-effects; considering an alternative treatment due to comorbidities; or simply needing to schedule a checkup to monitor health conditions and make further treatment decisions. Estimating the difference in outcomes between various actions one could follow based off such considerations, is a causal effect estimation question. Furthermore, this question involves several future treatment decisions taken at varying time points across our follow-up on the patient. Hence it is a sequential decision making problem. This type of data, where observations and treatments are given across time, appears in many applications. For instance in intensive care units, and in other domains like finance and social networks \citep{chen2021probabilistic, upadhyay2018deep}.

% Returning to our example of ASCVD prevention, to encourage a more informed and data-driven approach for this decision making, we need to take a closer look at the meaning of risk scores. For example, the notion of a 10-year risk score does not have a clear causal interpretation. It does not state whether the probabilities for heart disease are assessed assuming that no treatment is given, that the guidelines are followed, are any other treatment regime that might be relevant. To summarize, the interpretation of a risk score is contingent upon the assumptions about future treatments, which themselves influence the risk. Furthermore the treatment is not static \citep{chakraborty2014dynamic}; it may be revised upon the patient's future status and hence our risk score should help us understand how different treatment paths could alter that score. Therefore, to inform a decision about whether treatment can be delayed by a year, or revised in any of the aforementioned ways, we must asses its effect on the risk as entailed by future patient state and treatments. 

Formally, as we describe in \secref{sec:setting}, the problem falls within the framework of off-policy evaluation \citep{uehara2022review, fu2021benchmarks}. Differently from many applications in domains such as robotics and control, timings of treatment decisions and feature observations are irregularly spaced. These times must be accounted for in our algorithmic solutions, as they have a large effect on the outcome and we further wish to \emph{estimate the effect of intervening in treatment timing}. Trying to fit the problem into existing frameworks such as sequential decision making in discrete time results in several issues. For instance, time discretization can be inaccurate or inefficient, requiring us to make a choice about appropriate time scales for each dataset. Existing methods for continuous-time causal inference do not scale gracefully, since they solve complex estimation problems such as integrating importance weights across time \citep{roysland2011martingale}. Those that do scale to high capacity models and large datasets, do not handle dynamic policies (i.e. policies that take past states into account) and are implemented with differential equation solvers \citep{seedat2022continuous}, hence they do not solve the problem of interest and are inflexible in choice of architecture.


In this work we give two methods for off-policy evaluation with irregularly sampled data, a model we call a decision point process. Our contributions are as follows:
\begin{itemize}
    \item We define off-policy evaluation with decision point processes and develop \ours{}, a model-free solution to the problem. While other methods require computations that are intractable in high dimensions, or are limited to effect estimation of static treatments, \ours{} alleviates these caveats. It is based on direct regressions and dynamic programming, which makes it easily applicable to flexible architectures including sequence models such as transformers. We summarize related methods for scalable sequential treatment effect estimation in \Cref{tbl:related_methods} and explain the differences from this work.
 %    summarizes related estimation methods and their features.the developed method can be easily applied  
 % and does not require probabilistic modelling of future covariates, importance weights, nor differential equation solvers \citep{seedat2022continuous}. 
    
    \item In \Cref{thm:expectation_identity} we prove that \ours{} is an empirical estimator of the correct policy value. The estimator produces an accurate causal effect under assumptions on causal validity based on \citet{roysland2011martingale, roysland2022graphical}.
    % \textbf{TODO:} write down a lemma that states validity of the estimand $\E_{\lambda, \pi}[Y \vert \gH_t]$ and reference it here.
    \item An experimental demonstration on a time-to-failure prediction task for which we implement a transformer based solution, validates the efficacy of \ours{} where baselines that discretize time are suboptimal.
\end{itemize}

We define the effect estimation problem in \cref{sec:setting} using the formalism of temporal point processes, and discuss realted work in \cref{sec:related_work}. The solution is developed and validated experimentally in \cref{sec:method} and \cref{sec:experiments} respectively.
% Namely, the question of interest is in fact causal effect estimation.

% The American Heart Association guidelines advise on administering treatment when the $10$-year risk of heart failure is above !@!@!, which should render decision making simple. That is, we need to calculate of the risk scores developed in the past, and act accordingly to the result. However, matters are usually not that simple. For starters, a $10$-year risk score is ill-defined as it is only meaningful if we specify the course of future treatment (e.g. we could calculate the score under the assumption that no treatment will be provided in the future), since that treatment can affect the score. Another crucial aspect of the problem is that we usually care about the difference in risk scores when calculated over alternative treatments. For instance, it seems undesirable to put a patient on a treatment regime if the treatment has no effect on the risk score, compared to a no-treatment baseline. Moreover, some patients prefer taking treatment only if it has a very high chance of being effective, while others tend to get treatment even for smaller potential gains. This is one of the reasons why the medical community endorses ``shared decision making".

% Sequential decision making is ubiquitous across various domains, including healthcare, finance, and beyond. In hospitals, medical professionals administer treatments based on the evolving observations of a patient's condition; in financial markets, traders execute orders based on sequential information flows. Algorithmic decision support systems, therefore, play a pivotal role in enhancing the efficiency and effectiveness of such decisions. The essence of these systems often revolves around answering causal questions, which are fundamental to predicting and influencing outcomes.

% Consider the scenario of a doctor and a patient deliberating over a preventative treatment strategy for heart failure. According to the guidelines of the American Heart Association, treatment is recommended if the 10-year risk of heart failure exceeds a certain threshold. At first glance, this might seem straightforward—calculate the risk score using existing models and proceed based on the result. However, the reality is far more complex. The notion of a 10-year risk score, for example, is contingent upon the assumptions about future treatments, which themselves influence the risk. It's not just about computing a static score; it's about understanding how different treatment paths could alter that score.

% Moreover, the relative changes in risk scores under various treatment scenarios are critical. It would be impractical to recommend a treatment that does not modify the risk score compared to a no-treatment baseline. Furthermore, patient preferences play a crucial role; some patients might opt for treatment only if it significantly decreases their risk, whereas others might be willing to undergo treatment for even marginal improvements. This diversity in patient values and expectations underscores the importance of shared decision making in the medical field, where decisions are tailored to the individual's risk profile and treatment outlook.

% Thus, to truly support decision making in medicine and beyond, we must delve deeper into the causal mechanisms that govern the outcomes of our choices, ensuring that our algorithms can adapt to and effectively model these complex, dynamic scenarios.
